QCD field-strength correlators on a Polyakov loop with gradient flow at next-to-leading order

Momentum exchange between a heavy quark and a hot quark-gluon medium can be characterized nonperturbatively in terms of field-strength field-strength (E-E and B-B) correlators along a Polyakov loop. These can be studied on the lattice and analytically continued. However the lattice typically determines the correlators after the application of gradient flow. We investigate how gradient flow renormalizes these correlation functions by carrying out a next-to-leading order perturbative analysis of the correlators including gradient flow. This establishes a next-to-leading order renormalization matching between the correlators as measured on the lattice and the correlators relevant for momentum diffusion.

==> extrastuff.tex <==


, see Table \ref{Table of comparison quarkonium flowed}.
These results could be used in numerical evaluations, such as Ref.~\cite{Leino:2024pen}, to try to subtract known $\tauf$-dependent perimeter-law effects.

\begin{widetext}

\begin{table}[H]
\centering{}%
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
 & \multicolumn{3}{c|}{EE Correlator} &
 \multicolumn{3}{c|}{BB Correlator}
% & \multicolumn{1}{c}{Correlator} &
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{BB-Correlator} & 
 \tabularnewline[0.5ex]
\hline 
$\vphantom{\bigg|}$
Diagram & $\ln\left(\chi\right)+\gamma_{E}$ & $2\sqrt{\pi\chi}$ & Constant &  $\ln\left(\chi\right)+\gamma_{E}$ & $2\sqrt{\pi\chi}$ & Constant\tabularnewline[0.5ex]
\hline 
$b-f$ & $2$ & $-2$ & $4$ & $2$ & $-2$ & $4$\tabularnewline
\hline 
$g$ & 0 & $1$ & $-1$ & 0 & 0 & 0\tabularnewline
\hline 
$j_{1}$ & $3$ & $-\frac{4}{3}$ & $1+\frac{4}{3}\pi^{2}$ & $1$ & 0 & $5+\frac{4}{3}\pi^{2}$\tabularnewline[0.1cm]
\hline 
$j_{2}$ & 0 & $\frac{2}{3}$ & $\frac{5}{2}$ & 0 & 0 & 0\tabularnewline[0.1cm]
\hline 
$j_{3}$ & 0 & $-\frac{1}{3}$ & $-\frac{3}{8}$ & 0 & 0 & $\frac{1}{8}$\tabularnewline[0.1cm]
\hline 
\end{tabular}
\caption{Diagrams which must be reanalyzed for adjoint Wilson lines, with the new results, in the $\chi \gg 1$ limit.
Each value is multiplied by  $-g_{B}^{4}\CA\CR T_{F}/\left(2\pi\tau\right)^{4}N_{c}$.
}
\label{Table of comparison quarkonium flowed}
\end{table}

For none of the correlators of the $\MSBAR$ scheme changes exist, but an overall factor of $-T_{F}/N_{c}$. The changes within the flowed correlators at NLO due to the adjoint line are shown as follows:

\begin{align}
\label{GEadjflow}
G_{\mathrm{E,{adj}}}^{\mathrm{{flow}},\bar{\mu}}\left(\tau\right) & 
=- \frac{T_{F}}{N_{c}} \left(\GE^{\mathrm{{flow}},\bar{\mu}}\left(\tau\right) -\frac{g^4 \CR \CA}{\left(2\pi\tau\right)^{4}}\tau\sqrt{\frac{2\pi}{\tauf}}\right) 
\\
\label{GBadjflow}
G_{\mathrm{B,{adj}}}^{\mathrm{{flow}},\bar{\mu}}\left(\tau\right) & 
=- \frac{T_{F}}{N_{c}} \left(\GB^{\mathrm{{flow}},\bar{\mu}}\left(\tau\right) -\frac{g^4 \CR \CA}{\left(2\pi\tau\right)^{4}}\tau\sqrt{\frac{2\pi}{\tauf}}\right) 
\end{align}

\end{widetext}



==> propagator.tex <==
We find it by Fourier transforming the momentum-space expression:
\begin{align}
    & \Delta \left(x-y\right)_{s_1+s_2} 
    \\ & \equiv
    \int_{p}e^{ip\cdot(x-y)} \frac{e^{-(s_1+s_2)p^{2}}}{p^{2}}
\nonumber \\
    & = \frac{2^{D-2}}{(x-y)^{D-2} \left(4\pi\right)^{D/2}}
    \left(
    \Gamma \left(\textstyle{\frac D2}-1 \right)
    - \Gamma\left( \textstyle{\frac D2 -1 ,
    \frac{(x-y)^2}{4(s_1+s_2)}} \right) \right)
    \nonumber \\ \nonumber
    & \Rightarrow_{D=4}
    \frac{1}{4\pi^2 (x-y)^2} 
    \left( 1 - e^{-(x-y)^2/2(s_1+s_2)}  \right) .
\end{align}
Here $\Gamma(x)$ is the usual gamma function and $\Gamma(x,y)$ is the incomplete gamma function.
Since we will generally be interested in the case $(x-y)^2 \gg 4(s_1+s_2)$, we can often drop the incomplete gamma function, which leads to exponentially small corrections in this regime, as we see above for the case of 4 spacetime dimensions.






The first step in our renormalization procedure appears with the relation between the bare correlator and the $\MSBAR$ correlator where $Z_{b_{E}}$ and $Z_{b_{B}}$ are the renormalization factors for the color-electric correlator and the color-magnetic correlator, respectively. 
\[
\begin{array}{c}
    G_{E}^{\overline{\mbox{\scriptsize{MS}}},\bar{\mu}}\left(\tau\right)=Z_{{b_{E}}}^{2} G_{E}^{\mbox{\scriptsize{b}},\bar{\mu}}\left(\tau\right)=\left(1+\mathcal{O}\left(g^{4}\right)\right)^{2}G_{E}^{\mbox{\scriptsize{b}},\bar{\mu}}\left(\tau\right),
 \\
  \\
     G_{B}^{\overline{\mbox{\scriptsize{MS}}},\bar{\mu}}\left(\tau\right)=Z_{{b_{B}}}^{2} G_{B}^{\mbox{\scriptsize{b}},\bar{\mu}}\left(\tau\right)=\left(1+\frac{g^{2}\CA}{\left(4\pi\right)^{2}\epsilon}+\mathcal{O}\left(g^{4}\right)\right)^{2}G_{B}^{\mbox{\scriptsize{b}},\bar{\mu}}\left(\tau\right).
\end{array}
\]
